Design of Dual-Band Plasmonic Absorber for Biomedical Sensing and Environmental Monitoring

This study introduces a dual-band plasmonic absorber designed for simultaneous sensing applications in the near-infrared (NIR) and mid-infrared (MIR) regions. The absorber, composed of silver nanostructures on a metal plate with a dielectric spacer, exhibits a combination of localized and gap surface plasmon resonances, resulting in two distinct absorption peaks in theoretical analysis based on the FDTD method. Numerical simulations also validate the sensor's high refractive index sensitivity, enabling the detection of biomolecules, proteins, viruses, and various solutes in aqueous solutions. The absorber demonstrates significant resonance shifts, making it a promising candidate for environmental monitoring, medical diagnostics, and chemical sensing.

==> highlights_and_graphical_abstract.tex <==
\begin{graphicalabstract}

    \centering
    \includegraphics[width=1\textwidth]{Figures/Graphical Abstract/Graphical-abstract.pdf}
    \label{fig:Fig-Graphical-abstract}

\end{graphicalabstract}

\begin{highlights}
\item The article presents a dual-band plasmonic absorber for simultaneous sensing applications in the near-infrared (NIR) and mid-infrared (MIR) regions.
\item By leveraging localized surface plasmon resonances (LSPR) and gap surface plasmons (GSP) within the metal-dielectric-metal structure, the absorber achieves enhanced responsiveness to changes in refractive index.
\item With high sensitivity in two IR spectral regions, the absorber offers versatility for a range of uses, including effective environmental monitoring, medical diagnostics, and chemical sensing applications.
\end{highlights}
